Driving from Vision through Differentiable Optimal Control

This paper proposes DriViDOC: a framework for Driving from Vision through Differentiable Optimal Control, and its application to learn autonomous driving controllers from human demonstrations. DriViDOC combines the automatic inference of relevant features from camera frames with the properties of nonlinear model predictive control (NMPC), such as constraint satisfaction. Our approach leverages the differentiability of parametric NMPC, allowing for end-to-end learning of the driving model from images to control. The model is trained on an offline dataset comprising various human demonstrations collected on a motion-base driving simulator. During online testing, the model demonstrates successful imitation of different driving styles, and the interpreted NMPC parameters provide insights into the achievement of specific driving behaviors. Our experimental results show that DriViDOC outperforms other methods involving NMPC and neural networks, exhibiting an average improvement of 20% in imitation scores.

==> features.tex <==
\begin{table*}
	\centering
	\caption{NOIMG Baselines: performance metrics of the driving models for each driver. Less optimal results (Mean Z-score $>$ 2) are highlighted with a red color. The rows with a grey background correspond to the drivers with convergence to a high BC loss, who are excluded from average computations.}
	\label{tab:alldrivers_noimg}
\begin{tabular}{cllllllll}
\hline
\multicolumn{1}{l}{} & \multicolumn{2}{c}{$d$}                                    & \multicolumn{2}{c}{$v_x$}                                    & \multicolumn{2}{c}{\textbf{$a_x$}}                             & \multicolumn{2}{c}{$a_y$}                                      \\ \hline
\multicolumn{1}{l}{} & \multicolumn{1}{c}{AE $[m]$} & \multicolumn{1}{c}{Z-score} & \multicolumn{1}{c}{AE $[m/s]$} & \multicolumn{1}{c}{Z-score} & \multicolumn{1}{c}{AE $[m/s^2]$} & \multicolumn{1}{c}{Z-score} & \multicolumn{1}{c}{AE $[m/s^2]$} & \multicolumn{1}{c}{Z-score} \\ \hline
\rowcolor[HTML]{C0C0C0} 
Model00              & $1.60 \pm 0.39$              & $\textcolor{red}{7.91 \pm 4.20}$    & $13.67 \pm 2.30$               & $\textcolor{red}{30.38 \pm 9.85}$   & $0.14 \pm 0.21$                  & $\textcolor{red}{2.69 \pm 1.88}$    & $2.55 \pm 1.67$                  & $\textcolor{red}{8.97 \pm 7.38}$    \\ \hline
\rowcolor[HTML]{C0C0C0} 
Model01              & $1.75 \pm 0.58$              & $\textcolor{red}{4.71 \pm 2.95}$    & $12.21 \pm 2.26$               & $\textcolor{red}{14.36 \pm 7.50}$   & $0.34 \pm 0.26$                  & $1.49 \pm 2.47$             & $2.16 \pm 1.32$                  & $\textcolor{red}{4.62 \pm 3.37}$    \\ \hline
Model02              & $0.15 \pm 0.13$              & $1.04 \pm 1.01$             & $4.11 \pm 0.70$                & $\textcolor{red}{2.04 \pm 0.74}$    & $0.24 \pm 0.16$                  & $1.03 \pm 0.74$             & $1.00 \pm 0.70$                  & $1.96 \pm 1.27$             \\ \hline
Model03              & $0.31 \pm 0.25$              & $1.34 \pm 1.44$             & $1.73 \pm 0.97$                & $1.65 \pm 0.97$             & $0.43 \pm 0.31$                  & $\textcolor{red}{5.26 \pm 9.36}$    & $0.62 \pm 0.47$                  & $1.35 \pm 0.95$             \\ \hline
Model04              & $0.24 \pm 0.23$              & $0.93 \pm 0.87$             & $1.49 \pm 1.38$                & $1.61 \pm 1.57$             & $0.57 \pm 0.48$                  & $\textcolor{red}{2.33 \pm 2.19}$    & $0.63 \pm 0.48$                  & $1.64 \pm 1.23$             \\ \hline
Model05              & $0.52 \pm 0.37$              & $\textcolor{red}{3.01 \pm 2.80}$    & $2.09 \pm 1.42$                & $1.86 \pm 1.64$             & $0.29 \pm 0.23$                  & $0.81 \pm 0.68$             & $0.35 \pm 0.27$                  & $1.30 \pm 1.09$             \\ \hline
Model06              & $0.28 \pm 0.27$              & $0.90 \pm 1.11$             & $3.27 \pm 2.11$                & $1.73 \pm 1.42$             & $0.23 \pm 0.17$                  & $1.00 \pm 1.03$             & $0.68 \pm 0.67$                  & $1.53 \pm 1.68$             \\ \hline
Model07              & $0.31 \pm 0.29$              & $1.31 \pm 1.28$             & $3.15 \pm 1.62$                & $\textcolor{red}{2.30 \pm 1.33}$    & $0.33 \pm 0.25$                  & $2.00 \pm 2.62$             & $0.65 \pm 0.51$                  & $1.50 \pm 1.16$             \\ \hline
\rowcolor[HTML]{C0C0C0} 
Model08              & $1.48 \pm 0.54$              & $\textcolor{red}{3.55 \pm 1.95}$    & $13.65 \pm 2.62$               & $\textcolor{red}{14.14 \pm 6.51}$   & $0.43 \pm 0.25$                  & $\textcolor{red}{2.98 \pm 3.40}$    & $2.56 \pm 1.40$                  & $\textcolor{red}{5.23 \pm 3.46}$    \\ \hline
\rowcolor[HTML]{C0C0C0} 
Model09              & $1.57 \pm 0.58$              & $\textcolor{red}{5.41 \pm 4.07}$    & $12.53 \pm 2.18$               & $\textcolor{red}{24.69 \pm 14.27}$  & $0.17 \pm 0.19$                  & $1.43 \pm 1.53$             & $2.32 \pm 1.40$                  & $\textcolor{red}{7.88 \pm 6.42}$    \\ \hline
Model10              & $0.22 \pm 0.15$              & $1.30 \pm 1.13$             & $1.88 \pm 1.24$                & $1.50 \pm 1.25$             & $0.43 \pm 0.32$                  & $1.94 \pm 3.80$             & $0.60 \pm 0.51$                  & $1.30 \pm 1.15$             \\ \hline
\end{tabular}
\end{table*}

==> sf.tex <==
\begin{table*}
	\centering
	\caption{SF Baseline: performance metrics of the driving models for each driver. Less optimal results (Mean Z-score $>$ 2) are highlighted with a red colour.}
	\label{tab:alldrivers_sf}
	\begin{tabular}{cllllllll}
		\hline
		\multicolumn{1}{l}{} & \multicolumn{2}{c}{$d$}                                    & \multicolumn{2}{c}{$v_x$}                                    & \multicolumn{2}{c}{$a_x$}                                      & \multicolumn{2}{c}{$a_y$}                                      \\ \hline
		\multicolumn{1}{l}{} & \multicolumn{1}{c}{AE $[m]$} & \multicolumn{1}{c}{Z-score} & \multicolumn{1}{c}{AE $[m/s]$} & \multicolumn{1}{c}{Z-score} & \multicolumn{1}{c}{AE $[m/s^2]$} & \multicolumn{1}{c}{Z-score} & \multicolumn{1}{c}{AE $[m/s^2]$} & \multicolumn{1}{c}{Z-score} \\ \hline
		Model00 & $0.35 \pm 0.22$ & $1.73 \pm 1.58$ & $0.55 \pm 0.36$ & $1.18 \pm 0.72$ & $0.04 \pm 0.11$ & $0.75 \pm 0.71$ & $0.28 \pm 0.22$ & $0.99 \pm 0.89$ \\ \hline
		Model01 & $0.59 \pm 0.40$ & $1.71 \pm 1.68$ & $2.38 \pm 2.02$ & $\textcolor{red}{2.91 \pm 3.12}$ & $0.34 \pm 0.27$ & $0.95 \pm 0.94$ & $0.72 \pm 0.61$ & $1.64 \pm 1.61$ \\ \hline
		Model02 & $0.46 \pm 0.33$ & $\textcolor{red}{3.18 \pm 2.77}$ & $1.17 \pm 0.74$ & $0.55 \pm 0.31$ & $0.18 \pm 0.15$ & $0.71 \pm 0.69$ & $0.33 \pm 0.26$ & $0.83 \pm 1.00$ \\ \hline
		Model03 & $0.73 \pm 0.54$ & $\textcolor{red}{3.14 \pm 3.12}$ & $1.16 \pm 0.89$ & $1.12 \pm 0.90$ & $0.29 \pm 0.29$ & $\textcolor{red}{2.65 \pm 6.66}$ & $0.64 \pm 0.82$ & $1.45 \pm 1.80$ \\ \hline
		Model04 & $0.44 \pm 0.29$ & $1.85 \pm 1.45$ & $1.24 \pm 1.08$ & $1.28 \pm 1.10$ & $0.45 \pm 0.49$ & $1.26 \pm 1.35$ & $0.51 \pm 0.46$ & $1.35 \pm 1.25$ \\ \hline
		Model05 & $0.61 \pm 0.37$ & $\textcolor{red}{3.76 \pm 3.92}$ & $4.26 \pm 1.63$ & $\textcolor{red}{3.90 \pm 2.05}$ & $0.27 \pm 0.22$ & $0.78 \pm 0.76$ & $0.74 \pm 0.53$ & $\textcolor{red}{2.40 \pm 1.60}$ \\ \hline
		Model06 & $0.64 \pm 0.41$ & $\textcolor{red}{2.11 \pm 1.86}$ & $4.48 \pm 2.48$ & $\textcolor{red}{2.21 \pm 1.34}$ & $0.25 \pm 0.21$ & $1.02 \pm 1.04$ & $0.76 \pm 0.61$ & $1.50 \pm 1.10$ \\ \hline
		Model07 & $0.55 \pm 0.41$ & $\textcolor{red}{2.28 \pm 1.97}$ & $1.61 \pm 1.17$ & $1.17 \pm 0.94$ & $0.22 \pm 0.21$ & $0.86 \pm 0.87$ & $0.46 \pm 0.37$ & $1.08 \pm 0.94$ \\ \hline
		Model08 & $0.86 \pm 0.53$ & $\textcolor{red}{2.06 \pm 1.41}$ & $6.85 \pm 3.66$ & $\textcolor{red}{7.15 \pm 4.91}$ & $0.34 \pm 0.28$ & $\textcolor{red}{2.63 \pm 5.84}$ & $1.63 \pm 1.08$ & $\textcolor{red}{3.54 \pm 2.52}$ \\ \hline
		Model09 & $0.53 \pm 0.37$ & $1.87 \pm 1.79$ & $0.54 \pm 0.34$ & $1.04 \pm 0.90$ & $0.09 \pm 0.13$ & $0.54 \pm 0.46$ & $0.30 \pm 0.25$ & $0.95 \pm 0.82$ \\ \hline
		Model10 & $0.71 \pm 0.54$ & $\textcolor{red}{3.93 \pm 3.67}$ & $4.55 \pm 2.49$ & $\textcolor{red}{3.44 \pm 2.08}$ & $0.29 \pm 0.23$ & $1.07 \pm 1.04$ & $0.96 \pm 0.67$ & $1.90 \pm 1.20$ \\ \hline
	\end{tabular}
\end{table*}

==> track.tex <==
\begin{table*}
	\centering
	\caption{TRACK Baseline: performance metrics of the driving models for each driver. Less optimal results (Mean Z-score $>$ 2) are highlighted with a red colour.}
	\label{tab:alldrivers_track}
 	\begin{tabular}{cllllllll}
		\hline
		\multicolumn{1}{l}{} & \multicolumn{2}{c}{$d$}                                    & \multicolumn{2}{c}{$v_x$}                                    & \multicolumn{2}{c}{$a_x$}                                      & \multicolumn{2}{c}{$a_y$}                                      \\ \hline
		\multicolumn{1}{l}{} & \multicolumn{1}{c}{AE $[m]$} & \multicolumn{1}{c}{Z-score} & \multicolumn{1}{c}{AE $[m/s]$} & \multicolumn{1}{c}{Z-score} & \multicolumn{1}{c}{AE $[m/s^2]$} & \multicolumn{1}{c}{Z-score} & \multicolumn{1}{c}{AE $[m/s^2]$} & \multicolumn{1}{c}{Z-score} \\ \hline
		Model00 & $0.20 \pm 0.15$ & $0.96 \pm 0.84$ & $0.78 \pm 0.40$ & $1.53 \pm 0.81$ & $0.20 \pm 0.18$ & $\textcolor{red}{4.60 \pm 4.38}$ & $0.38 \pm 0.29$ & $1.29 \pm 0.99$ \\ \hline
		Model01 & $0.39 \pm 0.30$ & $1.07 \pm 0.99$ & $0.83 \pm 0.61$ & $0.95 \pm 0.89$ & $0.36 \pm 0.28$ & $1.36 \pm 1.73$ & $0.39 \pm 0.32$ & $0.94 \pm 0.89$ \\ \hline
		Model02 & $0.18 \pm 0.14$ & $1.19 \pm 0.99$ & $2.05 \pm 1.18$ & $1.01 \pm 0.66$ & $0.43 \pm 0.31$ & $1.76 \pm 1.41$ & $0.67 \pm 0.55$ & $1.52 \pm 1.25$ \\ \hline
		Model03 & $0.52 \pm 0.37$ & $\textcolor{red}{2.32 \pm 2.59}$ & $0.67 \pm 0.55$ & $0.62 \pm 0.55$ & $0.40 \pm 0.37$ & $\textcolor{red}{3.53 \pm 6.59}$ & $0.52 \pm 0.36$ & $1.36 \pm 1.34$ \\ \hline
		Model04 & $0.41 \pm 0.38$ & $1.58 \pm 1.67$ & $1.69 \pm 0.89$ & $1.88 \pm 1.22$ & $0.76 \pm 0.60$ & $\textcolor{red}{3.42 \pm 2.94}$ & $0.61 \pm 0.55$ & $1.75 \pm 2.16$ \\ \hline
		Model05 & $0.23 \pm 0.18$ & $1.36 \pm 1.41$ & $1.03 \pm 0.91$ & $1.13 \pm 1.03$ & $0.35 \pm 0.28$ & $1.13 \pm 1.29$ & $0.27 \pm 0.23$ & $1.03 \pm 0.91$ \\ \hline
		Model06 & $0.38 \pm 0.29$ & $0.94 \pm 0.76$ & $1.93 \pm 1.25$ & $1.03 \pm 0.83$ & $0.38 \pm 0.29$ & $1.68 \pm 1.71$ & $0.39 \pm 0.32$ & $0.96 \pm 0.99$ \\ \hline
		Model07 & $0.49 \pm 0.28$ & $\textcolor{red}{2.03 \pm 1.47}$ & $1.51 \pm 1.10$ & $1.09 \pm 0.89$ & $0.49 \pm 0.39$ & $\textcolor{red}{3.40 \pm 5.08}$ & $0.36 \pm 0.29$ & $0.92 \pm 0.82$ \\ \hline
		Model08 & $0.40 \pm 0.30$ & $0.96 \pm 0.76$ & $1.31 \pm 0.94$ & $1.20 \pm 0.95$ & $0.46 \pm 0.39$ & $\textcolor{red}{2.01 \pm 2.47}$ & $0.84 \pm 0.65$ & $1.91 \pm 1.73$ \\ \hline
		Model09 & $0.67 \pm 0.50$ & $\textcolor{red}{2.29 \pm 2.36}$ & $1.05 \pm 0.69$ & $\textcolor{red}{2.11 \pm 1.83}$ & $0.46 \pm 0.32$ & $\textcolor{red}{3.97 \pm 4.27}$ & $0.56 \pm 0.47$ & $1.94 \pm 2.02$ \\ \hline
		Model10 & $0.31 \pm 0.20$ & $1.74 \pm 1.56$ & $1.40 \pm 1.00$ & $1.17 \pm 1.17$ & $0.65 \pm 0.40$ & $\textcolor{red}{3.04 \pm 3.84}$ & $0.54 \pm 0.49$ & $1.25 \pm 1.49$ \\ \hline
	\end{tabular}
\end{table*}

==> ttests.tex <==
\begin{table}
	\centering
	\caption{Results of the one-tailed paired-sample t-test, validating increase on MAE and MZ for TRACK compared to DriViDOC. Statistically significant increases are highlighted in bold.}
	\label{tab:ttests_track}
 \resizebox{\columnwidth}{!}{
	\begin{tabular}{ccccc}
         & $d$ & $v_x$ & $a_x$ & $a_y$ \\
		\midrule
        MAE & p=0.514, stat=-0.04 & \textbf{p=0.017, stat=2.45} & \textbf{p=0.000, stat=7.10} & \textbf{p=0.011, stat=2.70}
        \\
        \midrule
        MZ & p=0.618, stat=-0.31 & \textbf{p=0.026, stat=2.21} & \textbf{p=0.000, stat=5.43} & \textbf{p=0.015, stat=2.54}
        \\
	\end{tabular}}
\end{table}


\begin{table}
	\centering
	\caption{Results of the one-tailed paired-sample t-test, validating increase on MAE and MZ for SF compared to DriViDOC. Statistically significant increases are highlighted in bold.}
	\label{tab:ttests_sf}
 \resizebox{\columnwidth}{!}{
	\begin{tabular}{ccccc}
        & $d$ & $v_x$ & $a_x$ & $a_y$ \\
		\midrule
    MAE & \textbf{p=0.001, stat=3.97} & \textbf{p=0.012, stat=2.65} & p=0.158, stat=1.05 & \textbf{p=0.018, stat=2.43}
    \\
    \midrule
    MZ & \textbf{p=0.002, stat=3.65} & \textbf{p=0.017, stat=2.46} & p=0.464, stat=0.09 & \textbf{p=0.023, stat=2.28}
    \\
	\end{tabular}}
\end{table}


\begin{table}
	\centering
	\caption{Results of the one-tailed paired-sample t-test, validating increase on MAE and MZ for NOIMG compared to DriViDOC. Models trained on drivers 00,03,10 and 11 have been excluded from the test (see main text). Statistically significant increases are highlighted in bold.}
	\label{tab:ttests_noimg}
 \resizebox{\columnwidth}{!}{
	\begin{tabular}{ccccc}
    & $d$ & $v_x$ & $a_x$ & $a_y$ \\
		\midrule
    MAE & p=0.897, stat=-1.42 & \textbf{p=0.006, stat=3.53} & \textbf{p=0.011, stat=3.07} & \textbf{p=0.004, stat=3.89}
    \\
    \midrule
    MZ & p=0.837, stat=-1.07 & \textbf{p=0.005, stat=3.64} & \textbf{p=0.037, stat=2.15} & \textbf{p=0.007, stat=3.48}
    \\
	\end{tabular}}
\end{table}
